Atomicity and Factorization of Puiseux Monoids

A Puiseux monoid is an additive submonoid of the nonnegative cone of rational numbers. Although Puiseux monoids are torsion-free rank-one monoids, their atomic structure is rich and highly complex. For this reason, they have been important objects to construct crucial examples in commutative algebra and factorization theory. In 1974 Anne Grams used a Puiseux monoid to construct the first example of an atomic domain not satisfying the ACCP, disproving Cohn's conjecture that every atomic domain satisfies the ACCP. Even recently, Jim Coykendall and Felix Gotti have used Puiseux monoids to construct the first atomic monoids with monoid algebras (over a field) that are not atomic, answering a question posed by Robert Gilmer back in the 1980s. This dissertation is focused on the investigation of the atomic structure and factorization theory of Puiseux monoids. Here we established various sufficient conditions for a Puiseux monoid to be atomic (or satisfy the ACCP). We do the same for two of the most important atomic properties: the finite-factorization property and the bounded-factorization property. Then we compare these four atomic properties in the context of Puiseux monoids. This leads us to construct and study several classes of Puiseux monoids with distinct atomic structure. Our investigation provides sufficient evidence to believe that the class of Puiseux monoids is the simplest class with enough complexity to find monoids satisfying almost every fundamental atomic behavior.

==> bibliography.tex <==
% This setup has you inputting the bibliography manually, this can be done away with by using
% BiBTeX, but that has not been used/implemented in this template, so, you are free/encouraged
% to use it to make your life much easier, but we are still in the process of integrating BiBTeX
\begin{thebibliography}{100}
\pagestyle{plain}
\bibitem{book:guide}
The~Editorial Office of the Graduate School,
\newblock \emph{Guide for Preparing Theses and Dissertations},
\newblock The University of Florida, \emph{Revised} 1998.

\bibitem{abdulra.m.sheikh.auh.ea:94}
M.~Abdulrahan, A.~U.~H. Sheikh, and D.~D. Falconer,
\newblock ``Decision feedback equalization for {CDMA} in indoor wireless
  communications,''
\newblock \emph{IEEE Journal on Selected Areas in Communications}, vol. 12, no.
  4, pp. 698--706, May 1994.

\bibitem{barbosa.an.miller.sl:98}
A.~N. Barbosa and S.~L. Miller,
\newblock ``Adaptive detection of {DS/CDMA} signals in fading channels,''
\newblock \emph{IEEE Transactions on Communications}, vol. 46, no. 1, pp.
  115--124, Jan. 1998.

\bibitem{barghou.rt.stuber.gl:92}
R.~T. Barghouthi and G.~L. St{\"u}ber,
\newblock ``Sequence acquisition techniques for {CDMA} systems employing
  {Kasami} sequences,''
\newblock in \emph{Proceedings~IEEE Military Communications Conference}, San
  Diego, CA, 1992, vol.~2, pp. 633--637.

\bibitem{barghou.rt.stuber.gl:94}
R.~T. Barghouthi and G.~L. St{\"u}ber,
\newblock ``Rapid sequence acquisition for {DS/CDMA} systems employing {Kasami}
  sequences,''
\newblock \emph{IEEE Transactions on Communications}, vol. 42, no. 2/3/4, pp.
  1957--1968, Feb./Mar./Apr. 1994.

\bibitem{bensley.se.aazhang.b:96}
S.~E. Bensley and B.~Aazhang,
\newblock ``Subspace-based channel estimation for code division multiple access
  communication systems,''
\newblock \emph{IEEE Transactions on Communications}, vol. 44, no. 8, pp.
  1009--1020, Aug. 1996.

\bibitem{bensley.se.aazhang.b:98}
S.~E. Bensley and B.~Aazhang,
\newblock ``{Maximum}-{Likelihood} synchronization of a single user for
  code-division multiple-access communication systems,''
\newblock \emph{IEEE Transactions on Communications}, vol. 46, no. 3, pp.
  392--399, Mar. 1998.

\bibitem{bershad.nj.qu.lz:89}
N.~J. Bershad and L.~Z. Qu,
\newblock ``On the probability density function of the {LMS} adaptive filter
  weights,''
\newblock \emph{IEEE Transactions on Acoustics, Speech and Signal Processing},
  vol. 37, no. 1, pp. 43--56, Jan. 1989.

\bibitem{braun.wr:97}
W.~R. Braun,
\newblock ``{PN} acquisition and tracking performance in {DS/CDMA} systems with
  symbol-length spreading sequences,''
\newblock \emph{IEEE Transactions on Communications}, vol. 45, no. 12, pp.
  1595--1601, Dec. 1997.

\bibitem{buehrer.rm.kaul.a.ea:96}
R.~M. Buehrer, A.~Kaul, S.~Striglis, and B.~D. Woerner,
\newblock ``Analysis of {DS-CDMA} parallel interference cancellation with phase
  and timing errors,''
\newblock \emph{IEEE Journal on Selected Areas in Communications}, vol. 14, no.
  8, pp. 1522--1535, Oct. 1996.

\bibitem{buehrer.rm.woerner.bd:95}
R.~M. Buehrer and B.~D. Woerner,
\newblock ``Analysis of adaptive multistage interference cancellation for
  {CDMA} using an improved {Gaussian} approximation,''
\newblock in \emph{Proceedings~IEEE Military Communications Conference}, San
  Diego, CA, 1995, vol.~3, pp. 1195--1199.

\bibitem{chang.rw.sriniva.r:80}
R.~W. Chang and R.~Srinivasagopalan,
\newblock ``Carrier recovery for data communication systems with adaptive
  equalization,''
\newblock \emph{IEEE Transactions on Communications}, vol. COM--28, no. 8, pp.
  1142--1153, Aug. 1980.

\bibitem{clarke.rh:68}
R.~H. Clarke,
\newblock ``A statistical theory of mobile-radio reception,''
\newblock \emph{The Bell System Technical Journal}, vol. 47, no. 6, pp.
  957--1000, July-Aug. 1968.

\bibitem{couch-ii.lw:97}
L.~W. Couch~II,
\newblock \emph{Digital and Analog Communication Systems},
\newblock Prentice-Hall, 5th edition, 1997.

\bibitem{davies.rb:73}
R.~B. Davies,
\newblock ``Numerical inversion of a characteristic function,''
\newblock \emph{Biometrika}, vol. 60, no. 2, pp. 415--417, 1973.

\bibitem{davies.rb:80}
R.~B. Davies,
\newblock ``The distribution of a linear combination of $\chi^2$ random
  variables,''
\newblock \emph{Applied Statistics}, vol. 29, no. 3, pp. 323--333, 1980.

\bibitem{douglas.sc.meng.thy:92}
S.~C. Douglas and T.~H.-Y. Meng,
\newblock ``Exact expectation analysis of the {LMS} adaptive filter without the
  independence assumption,''
\newblock in \emph{Proceedings~IEEE International Conference on Acoustics,
  Speech and Signal Processing}, San Francisco, CA, 1992, vol.~4, pp. 61--64.

\bibitem{douglas.sc:93}
S.~C. Douglas,
\newblock ``Exact expectation analysis of the {LMS} adaptive filter for
  correlated {Gaussian} input data,''
\newblock in \emph{Proceedings~IEEE International Conference on Acoustics,
  Speech and Signal Processing}, Minneapolis, MN, 1993, vol.~3, pp. 519--522.

\end{thebibliography}


==> tex/TwoOrMoreAppendices.tex <==
% The Editorial Office Requirements for the Table of Contents cause a significant problem
%in Latex if there is only one Appendix. The Appendix is no longer labeled "A" in the TOC
%but has the word "APPENDIX" placed in front of the title of the Appendix. This can be done
%without issue IF nothing needs to be numbered by LaTeX in the Appendix. Unfortunately, most of the time
%something needs to be numbered in that single Appendix. For this reason we have included the IFTHENELSE switch
%found in this document and at the beginning of AppendixA. We assume that if you have any appendices, that you have more than one. However, you DO only have one appendix DO NOT USE THIS FILE!!!!!!!!!!!!!!!!!!!!!!!
%
% OneSingleAppendix.tex has all the settings needed to adjust for a single appendix
% you will have a major problem with your TOC if you use this file with a single appendix!!!!!

%
% Comment (or delete) all of the \input{AppendixB} commands except those you are using.
%Then open the AppendixA.tex file and continue there.

%you can add/substract individual appendices through by using the /include{appendix'X'}
% and creating/deleting the appropriate files
\appendix %
%\clearpage%

\addtocontents{toc}{\protect\addvspace{10pt}\noindent{APPENDIX} \protect\hfill\par}{}
\setcounter{equation}{0}

\input{tex/appendixA} %
%\input{tex/appendixE} % %These files aren't included in the template
%\input{tex/appendixF} %
%\input{appendix/appendixC}
%\input{appendix/appendixD}
%\input{appendix/appendixE}


==> tex/abbreviations.tex <==
%%-----------List of Symbols, Nomenclature or Abbreviation--------

%% Please note: a list of Symbols, terms, acronyms, etc. is not usually the best practice.
%% More often you should simply define an abbreviation the first time it is used.
%% If you DO need to include a list like this please notice that it must be paginated manually
%% by breaking it up into page size tables. Longtable will not wrap the definition properly if
%% it extends to a second line and a similar issue is encountered when the tabbing environment
%% is used. If you have a better way of meeting the Editorial Office requirements I'd love to hear about it.

\chapter*{LIST OF SYMBOLS, NOMENCLATURE, OR ABBREVIATIONS} \addcontentsline{toc}{chapter}{LIST OF SYMBOLS} %Start
%writing here. This is optional.
\singlespacing
\begin{tabular}{l p{5in}} %if the terms in the first column are longer than 1.4 inches reduce the number 5 appropriately
$\sum$ & Denotes the summation of a series of terms\\
\\%This adds the single space between definitions (required)
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\

\end{tabular}

\begin{tabular}{lp{5in}}
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
$\sum$ & Denotes the summation of a series of terms\\
\\
$\bigcap$ & A really big bigcap\\
\\
fractal & A geometric pattern that is repeated at ever smaller
scales to produce irregular shapes and surfaces that cannot be represented by classical
geometry. Fractals are used especially in computer modeling of irregular patterns and structures in nature.}\\
\\
polynomial & (in one variable) an expression consisting of the sum of two
or more terms each of which is the product of a constant and a
variable raised to an integral power: $ax^2 + bx + c$ is a
polynomial, where $a, b,$ and $c$ are constants and $x$ is a
variable.}\\
\\
\end{tabular}
\doublespacing


